HICO-DET-SG and V-COCO-SG: New Data Splits for Evaluating the Systematic Generalization Performance of Human-Object Interaction Detection Models

Human-Object Interaction (HOI) detection is a task to localize humans and objects in an image and predict the interactions in human-object pairs. In real-world scenarios, HOI detection models need systematic generalization, i.e., generalization to novel combinations of objects and interactions, because the train data are expected to cover a limited portion of all possible combinations. To evaluate the systematic generalization performance of HOI detection models, we created two new sets of HOI detection data splits named HICO-DET-SG and V-COCO-SG based on the HICO-DET and V-COCO datasets, respectively. When evaluated on the new data splits, HOI detection models with various characteristics performed much more poorly than when evaluated on the original splits. This shows that systematic generalization is a challenging goal in HOI detection. By analyzing the evaluation results, we also gain insights for improving the systematic generalization performance and identify four possible future research directions. We hope that our new data splits and presented analysis will encourage further research on systematic generalization in HOI detection.

==> 2_related_old.tex <==
% \section{Related works}
% In section \ref{hoi methods}, we introduce some types of HOI detection models and datasets. In section \ref{sg in computer vision}, we explain systematic generalization in other computer tasks and similar problem settings to systematic generalization.

% \subsection{Human-Object Interaction (HOI) detection}
% \label{hoi methods}
% The task of HOI detection consists of two tasks. The first task is to localize humans and objects in the given image. The second one is to identify the interactions between them. 
% Due to this property, there are two types of model architectures to solve HOI detection: two-stage model and one-stage model. 
% Two-stage models~\citep{gao_2018,li_2019,Gao_2020,li_2020neurips,Liao_2022} detect humans and objects at the first stage and classify the relationship for all of their combinations in the second stage. In order to improve both instance and interaction detectors via multi-task learning and to reduce inference time, one-stage models~\citep{liao_2020,Gkioxari_2018} have been proposed recently and becoming more popular these days. In response to the great success of Transformer~\citep{Vaswani_2017} in both natural language processing and computer vision~\citep{Khan_2021}, some of the recent works~\citep{Kim_2021,Chen_2021,Tamura_2021,zhang_2021,chen_2021_Reformulating,Zou_2021} are based on Transformer as they are designed to capture wide-range information from an image.


% There are two popular datasets for HOI detection: HICO-DET and V-COCO datasets.
% HICO-DET dataset was originally created for classifying objects and interactions in the image (no bounding-box)~\citep{chao_2015}. Later they put bounding-boxes of humans and objects in the image~\citep{chao_2018}. Also, at this point, one image in the dataset can contain multiple humans, objects and interactions between them.
% Statistics of the HICO-DET dataset is shown in Table \ref{table_hico_stat}. There are 80 object, 117 interaction, and 600 object-interaction combination classes.

% V-COCO dataset~\citep{gupta_2015} was created based on Microsoft COCO (MS COCO) dataset~\citep{lin_2014} by adding annotations of verbs.
% Statistics of the V-COCO dataset is shown in Table \ref{table_vcoco_stat}. There are 80 object and 29 interaction classes and 228 combinations of object-interaction labels.

% \subsection{Systematic generalization in computer vision tasks}
% \label{sg in computer vision}
% Systematic generalization can be regarded as one of the Out-of Distribution (OoD) problem settings, i.e., the model needs to generalize to different data distributions from train data.

% In various computer vision tasks, generalization to OoD data is essential because it is known that the accuracy decreases in OoD situations. When applying a model to the real world, it is very likely to be an OoD situation because it requires processing data with a different distribution than the collected data in the training environment.

% In image classification tasks, OoD performance is tested on four datasets with various ratios of seen objects\citep{Sakai_2021}. It is proved that the diversity in train data leads to high systematic generalization performance\citep{Madan_2022}. Those works focus on Convolutional Neural Network (CNN) based models because they achieve state-of-the-art performances in image classification tasks.


% In Visual Question Answering (VQA) tasks, there are some types of OoD problem settings. Some of them require systematic generalization.
% Transformer-based Modular Network (TMN) is proposed to achieve state-of-the-art systematic generalization performance in three VQA datasets\citep{Yamada_2022}.


% In the HOI detection task, HICO-DET dataset~\citep{chao_2015,chao_2018} provides rare-triplets evaluation to measure the few-shot generalization ability of the models. Rare triplets are defined to appear less than 10 times in the train data. Some works~\citep{Baldassarre_2020,ji_2021} aims at improving especially rare-triplets accuracy.
% But there are no benchmarks or previous works to tackle systematic generalization, i.e., zero-shot generalization in HOI detection.




==> 4_experiments_old.tex <==
% \section{Experimental setup for evaluating representative HOI detection models}
% In this section, we describe the experiments to evaluate the systematic generalization ability of representative HOI detection models. In section \ref{methods}, we explain the evaluated models and the reasons for selecting those models. 

% \begin{table*}[htbp]
% \begin{center}
% \caption{Comparison of three HOI detection models, HOTR, QPIC, and QAHOI. We show mAPs (\%) on the original HICO-DET and V-COCO reported in the original papers; the higher, the better. ``HICO-DET (rare)'' shows the performance on rare triplets, i.e., few-shot generalization. The QAHOI paper does not report mAP on the V-COCO dataset.}
% {\small{
% \begin{tabular}{c|ccc}
% \hline 
%  & HOTR~\citep{Kim_2021} & QPIC~\citep{Tamura_2021} & QAHOI~\citep{Chen_2021} \\
% \hline 
% % \hline 
% Architecture type & One-stage parallel & One-stage end-to-end & One-stage end-to-end \\
% % \hline 
% Feature extractor & CNN & CNN & Multi-scale Transformer \\
% % \hline
% Base model & DETR~\citep{carion_2020} & DETR~\citep{carion_2020} & deformable DETR~\citep{zhu_2021} \\
% % \hline
% mAP on HICO-DET (full) & 25.73 & 29.90 & 35.78 \\
% % \hline 
% mAP on HICO-DET (rare) & 17.34 & 23.92 & 29.80 \\
% % \hline 
% mAP on V-COCO & 63.8 & 61.0 & - \\
% \hline
% \end{tabular}
% }}
% \end{center}
% \label{table_models}
% \end{table*}


% \subsection{HOI detection models}
% \label{methods}
% We tested systematic generalization performance for three HOI detection models. The comparison of the three models is shown in Table \ref{table_models}. The selected models are all one-stage architecture since they achieve much higher accuracies compared to two-stage models, which were popular previously.
% The backbone (feature extraction) network of each model is all trained with object detection tasks on MS COCO dataset~\citep{lin_2014}.
% Our experiments are based on codes from original githubs.

% \paragraph{HOTR.}
% ``Human-Object interaction detection TRansformer'' (HOTR)~\citep{Kim_2021} is the first Transformer-based model in the HOI detection task. The model is one-stage parallel architecture as it has a backbone, shared encoder, instance (human + object) decoder, and interaction decoder. 
% The backbone network is CNN-based to extract features from images.
% In order to get the matching between instance and interaction decoder outputs, three independent feed-forward networks, which are so-called HO-pointers, are prepared to estimate correct \textless human, interaction, object\textgreater \hspace{0mm} combination matching. 
% Most of the network except HO-pointers is based on ``DEtection TRansformer'' (DETR)~\citep{carion_2020}, a Transformer-based object detection model. Therefore we can pre-train backbone, shared encoder, instance decoder, and interaction decoder with the DETR's weights trained on the MS COCO dataset.
% \paragraph{QPIC.}
% ``Query-based Pairwise human-object interaction detection with Image-wide contextual information'' (QPIC)~\citep{Tamura_2021} is another HOI detection model, and it is also based on DETR for most of the network. The main difference between HOTR is that QPIC is a one-stage end-to-end architecture that has only one single decoder without HO-pointers. They achieve better performance than HOTR because they can train the decoder via multi-task learning. 
% We can use pre-trained weights of DETR on MS COCO datasets for most of the network, including backbone, encoder, and decoder.
% \paragraph{QAHOI.}
% ``Query-based Anchors for Human-Object Interaction detection'' (QAHOI)~\citep{Chen_2021} achieves the state-of-the-art performance in the HOI detection on HICO-DET dataset as of the submission time on Papers with Code\footnote{\url{https://paperswithcode.com/sota/human-object-interaction-detection-on-hico}}. 
% The model is based on deformable DETR~\citep{zhu_2021}, a modified DETR, which computes self-attention from a limited range of feature maps for computational efficiency. This enables to extract multi-scale feature maps from the image. 
% There is another technique to reduce computational costs in the encoder and decoder. The encoder is trained to generate query-based anchors which represent the points with high objectness score in the image. The decoder predicts objects and interactions only on those anchors for efficient computation.
% Although the backbone of the network can be pre-trained because it is based on Swin Transformer~\citep{Liu_2021}, it is impossible to pre-train all the encoder and decoder because there are some modifications to deformable DETR (object detection model).

% \subsection{Pre-training, hyperparameters, and other conditions}
% In order to evaluate all the models on the equal condition in terms of pre-training, we report results of HOTR and QPIC for both pre-trained and not pre-trained encoder and decoder, despite that the original papers encourage to use pre-trained weights for the best performance in the original HOI detection tasks.
% We note that for all of our experiments, the backbone of each model, i.e., feature extraction part, is pre-trained with the same weights as the original experiments. We do not conduct experiments regarding this condition because we consider all the three models are on the same condition about backbone pre-training.


% For all of the three models, we used almost the same hyperparameters as reported in the original papers and repositories. But we reduced the batch size of QAHOI from 2 to 1, because we got a memory error while training with the default setting.
% In addition, we trained QAHOI on V-COCO and V-COCO-SG with the same hyperparameters as HICO-DET and HICO-DET-SG, as the original paper does not report the hyperparameters on V-COCO dataset.

% We conducted all the experiments once, and one experiment takes about 1 to 2 days with 4 NVIDIA V100 GPUs.


==> 7_ack.tex <==
% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2022/PaperInformation/FundingDisclosure}.


% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}


==> 9_checklist.tex <==



\begin{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% {\color{blue} Note: Comment out this section at the submission time}



%\subsection*{NeurIPS 2022} % https://neurips.cc/Conferences/2022/PaperInformation/StyleFiles


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See the abstract and Section \ref{intro}}
  \item Did you describe the limitations of your work?
    \answerNo{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{But we don't discuss potential negative societal impacts of our work}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{But we are going to include codes for making our data splits}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section \ref{datasets} and Appendix \ref{app_b}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{But we randomly created three distinct data splits and ran the experiments once for each splits}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix \ref{settings}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section \ref{datasets}}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We are going to include URL of the codes to create data splits}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\begin{comment}

\subsection*{The Machine Learning Reproducibility Checklist ( v2.0, Apr.7 2020 )} % https://www.cs.mcgill.ca/~jpineau/ReproducibilityChecklist.pdf

For all models and algorithms presented, check if you include:
\begin{itemize}
\item[] $\CheckedBox$ A clear description of the mathematical setting, algorithm, and/or model.
\item[] $\CheckedBox$ A clear explanation of any assumptions.
\item[] $\CheckedBox$ An analysis of the complexity (time, space, sample size) of any algorithm.
\end{itemize}

For any theoretical claim, check if you include:
\begin{itemize}
\item[] $\CheckedBox$ A clear statement of the claim.
\item[] $\CheckedBox$ A complete proof of the claim.
\end{itemize}

For all datasets used, check if you include:
\begin{itemize}
\item[] $\CheckedBox$ The relevant statistics, such as number of examples.
\item[] $\CheckedBox$ The details of train / validation / test splits.
\item[] $\CheckedBox$ An explanation of any data that were excluded, and all pre-processing step.
\item[] $\Box$ A link to a downloadable version of the dataset or simulation environment.
\item[] $\CheckedBox$ For new data collected, a complete description of the data collection process, such as instructions to annotators and methods for quality control.
\end{itemize}

For all shared code related to this work, check if you include:
\begin{itemize}
\item[] $\Box$ Specification of dependencies.
\item[] $\CheckedBox$ Training code.
\item[] $\CheckedBox$ Evaluation code.
\item[] $\CheckedBox$ (Pre-)trained model(s).
\item[] $\Box$ README file includes table of results accompanied by precise command to run to produce
those results.
\end{itemize}

For all reported experimental results, check if you include:
\begin{itemize}
\item[] $\CheckedBox$ The range of hyper-parameters considered, method to select the best hyper-parameter
configuration, and specification of all hyper-parameters used to generate results.
\item[] $\CheckedBox$ The exact number of training and evaluation runs.
\item[] $\CheckedBox$ A clear definition of the specific measure or statistics used to report results.
\item[] $\Box$ A description of results with central tendency (e.g. mean) \& variation (e.g. error bars).
\item[] $\CheckedBox$ The average runtime for each result, or estimated energy cost.
\item[] $\CheckedBox$ A description of the computing infrastructure used.
\end{itemize}
\end{comment}

